DIAL: Deep Interactive and Active Learning for Semantic Segmentation in Remote Sensing

We propose in this article to build up a collaboration between a deep neural network and a human in the loop to swiftly obtain accurate segmentation maps of remote sensing images. In a nutshell, the agent iteratively interacts with the network to correct its initially flawed predictions. Concretely, these interactions are annotations representing the semantic labels. Our methodological contribution is twofold. First, we propose two interactive learning schemes to integrate user inputs into deep neural networks. The first one concatenates the annotations with the other network's inputs. The second one uses the annotations as a sparse ground-truth to retrain the network. Second, we propose an active learning strategy to guide the user towards the most relevant areas to annotate. To this purpose, we compare different state-of-the-art acquisition functions to evaluate the neural network uncertainty such as ConfidNet, entropy or ODIN. Through experiments on three remote sensing datasets, we show the effectiveness of the proposed methods. Notably, we show that active learning based on uncertainty estimation enables to quickly lead the user towards mistakes and that it is thus relevant to guide the user interventions.

==> codes/figures/scratch.tex <==
\begin{figure}[!h]
    \newcommand\x{.32}
    \scriptsize
    \begin{subfigure}[t]{\x\linewidth}
        \centering\epsfig{figure=figures/scratch/annots.png,width=\linewidth}
        \captionsetup{width=.95\linewidth}
        \caption{Target image with 6 annots/class}
        % \caption{}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\x\linewidth}
        \centering\epsfig{figure=figures/scratch/noise.png,width=\linewidth}
        \captionsetup{width=.95\linewidth}
        \caption{Noisy DISCA output}
        % \caption{}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\x\linewidth}
        \centering\epsfig{figure=figures/scratch/gt.png,width=\linewidth}
        \captionsetup{width=.95\linewidth}
        \caption{Ground-truth}
        % \caption{}
    \end{subfigure}
    	\caption{Training DISCA from scratch on few annotations.}
    \label{fig:scratch}
\end{figure}

==> codes/tables/results.tex <==
%%%%%%%%%%%%%%%%%%%%% WITHOUT ALCD
\begin{table}[ht]
\caption{Performances in terms of mean IoU before and after the interactive processes with 10 annotations per image.} %\hl{A modifier pour ajouter une colonne DIAL (qui utilise disca). Éventuellement une deuxieme qui utilise AC ? Ajouter aussi un paragraphe dans la partie set up qui explique comment j'évalue pour AC et disca "naifs". Autre problème: les performances random avec disca en mode dial sont vraiment très mauvaises ...}
\centering
\begin{tabular}{c|a|cc??cc}
\toprule % \multirow{2}{*}{\textit{Dataset}}
         &  \multicolumn{3}{c??}{\textbf{Mean IoU}} & \multicolumn{2}{c}{\textbf{$\Delta$ IoU}} \\
 & \textit{Initial}      & \textit{AC}      & \textit{DISCA}      & \textit{AC}          & \textit{DISCA}          \\ 
\midrule
\textit{ISPRS}   & 70.7         & 71.7       & \textbf{72.4}       & 1              & \textbf{1.7}            \\
\textit{INRIA}   & 85.4         & 86.4       & \textbf{86.5}       & 1              & \textbf{1.1}            \\
% \textit{AIRS}    & 85.9         & 89.5       & \textbf{90.6}       & 3.6            & \textbf{4.7}           \\
\textit{AIRS}    & 88         & 89.8       & \textbf{90.2}       & 1.8            & \textbf{2.2}           \\
\bottomrule
\end{tabular}
\label{tab:results}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% WITH ALCD
% \begin{table*}[h]
% \caption{Performances and gains of the interactive processes with 10 annotations.}
% \centering
% \begin{tabular}{c|ccccc??ccc}
% \toprule % \multirow{2}{*}{\textit{Dataset}}
%          &  \multicolumn{5}{c??}{\textbf{Mean IoU}} & \multicolumn{3}{c}{$\mathbf{\Delta}$\textbf{IoU}} \\
%  & \textit{Initial}      & \textit{AC}      & \textit{DISCA}   & $\textit{ALCD}_{\textit{ini}}$ & \textit{ALCD}   & \textit{AC}          & \textit{DISCA}    & \textit{ALCD}      \\ 
% \midrule
% \textit{ISPRS}   & 70.7         & 71.7       & \textbf{72.4}    &  30 & 30.2 & 1              & \textbf{1.7}    &        0.2\\
% \textit{INRIA}   & 85.4         & 86.4       & \textbf{86.5}    &  - & - & 1              & \textbf{1.1}       &     -\\
% \textit{AIRS}    & 85.9         & 89.5       & \textbf{90.6}    &  - & - & 3.6            & \textbf{4.7}       &    -\\
% \bottomrule
% \end{tabular}
% \label{tab:results}
% \end{table*}


